Denoised Self-Augmented Learning for Social Recommendation

Social recommendation is gaining increasing attention in various online applications, including e-commerce and online streaming, where social information is leveraged to improve user-item interaction modeling. Recently, Self-Supervised Learning (SSL) has proven to be remarkably effective in addressing data sparsity through augmented learning tasks. Inspired by this, researchers have attempted to incorporate SSL into social recommendation by supplementing the primary supervised task with social-aware self-supervised signals. However, social information can be unavoidably noisy in characterizing user preferences due to the ubiquitous presence of interest-irrelevant social connections, such as colleagues or classmates who do not share many common interests. To address this challenge, we propose a novel social recommender called the Denoised Self-Augmented Learning paradigm (DSL). Our model not only preserves helpful social relations to enhance user-item interaction modeling but also enables personalized cross-view knowledge transfer through adaptive semantic alignment in embedding space. Our experimental results on various recommendation benchmarks confirm the superiority of our DSL over state-of-the-art methods. We release our model implementation at: https://github.com/HKUDS/DSL.

==> relate.tex <==
\section{Related Work}
\label{sec:relate}



==> response.tex <==

% \section*{Response to Reviewers}

\noindent We would like to express our sincere appreciation to the reviewers for taking the time to review our manuscript and provide thoughtful comments and suggestions. We have carefully considered the provided comments and made revisions to address them in our paper accordingly. \\\vspace{-0.12in}

\noindent \textbf{\bf Response to Reviewer \#1}\\
Thanks the reviewer for the positive feedback and the acknowledgement of the contribution in this work. \\\vspace{-0.12in}

% We would like to thank the reviewer for their careful reading and helpful comments. We have revised the manuscript to address the questions raised by the reviewer.

\noindent \textbf{Comment 1}: Parameter tuning in Eq.(9).\\\vspace{-0.15in}

\noindent \textbf{Response}: In our \model\ method, we define a joint loss function in Eq.(9) which includes different terms, namely the ranking-based BPR loss, augmented self-supervised optimized objective, and regularization for model training. The weights of these loss terms, such as $\lambda_1$, $\lambda_2$, and $\lambda_3$, are fine-tuned in the range of (0,1) on different experimental datasets. The best performance is achieved on Ciao, Epinions, and Yelp, with specific settings ($\lambda_1= 1e^{-1}$, $\lambda_2= 1e^{-5}$, $\lambda_3= 1e^{-5}$), ($\lambda_1= 1e^{-2}$, $\lambda_2= 1e^{-5}$, $\lambda_3= 1e^{-5}$) and ($\lambda_1= 1e^{0}$, $\lambda_2= 1e^{-5}$, $\lambda_3= 1e^{-6}$), respectively. Detailed information regarding these settings can be found in our released implementation code. \\\vspace{-0.1in}

\noindent \textbf{\bf Response to Reviewer \#2}\\
Thank you for your review and valuable feedback. We are glad to know that you find our paper is clearly written and results are reproducible. \\\vspace{-0.15in}

\noindent \textbf{Comment 1}: Discussion on baseline selection.\\\vspace{-0.13in}

% Our set of baselines included: i) matrix factorization (MF)-based approaches (PMF and TrustMF); ii) attention-based approach (EATNN); iii) GNN-enhanced models (DiffNet, DGRec, and NGCF+); and iv) recently proposed self-supervised recommenders (MHCN, KCGN, SMIN, and DcRec).

\noindent \textbf{Response}: To provide a comprehensive evaluation of our DSL approach, we selected baseline models that represent different paradigms in social recommendation. These models are widely adopted as baselines for performance comparison in recent research works and are representative of various social recommendation approaches. For example, MHCN and SMIN are two newly proposed methods that provide state-of-the-art performance using self-supervised learning. \\\vspace{-0.12in}

\noindent \textbf{Comment 2}: Links to the datasets.\\\vspace{-0.12in}

\noindent \textbf{Response}: All the evaluation datasets have been updated in the anonymous repository with the corresponding details.\\\vspace{-0.12in}

\noindent \textbf{Comment 3}: Evaluation method justification.\\\vspace{-0.12in}

\noindent \textbf{Response}: To ensure fair comparison, we adopt the evaluation protocols similar to those used in ~\cite{wu2019neural,long2021social}. To enable efficient result evaluation, we pair the positive sample of the target user with 99 negative instances that have no prior interaction with the user. \\\vspace{-0.12in}

\noindent \textbf{Comment 4}: Clarification of user selection in case study.\\\vspace{-0.12in}

\noindent \textbf{Response}: We selected the user cases based on the learned user-wise relevance scores, where the top-10 and bottom-10 ranked user pairs were considered. Upon inspection, we observed that our learned user dependency scores could effectively capture most of the interaction similarities between these users. To improve our case study, we add more samples from the top-10 and bottom-10 ranked users in Figure~\ref{fig:new_case}.

\begin{figure}[htbp]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=0.45\textwidth]{figure/new_case_study.pdf}
    \vspace{-0.1in}
    \caption{Case study is conducted to evaluate the effectiveness of denoising social relations for modeling user-item interaction patterns.}
    \vspace{-0.1in}
    \label{fig:new_case}
\end{figure}

\noindent \textbf{Comment 5}: More background discussion on Section 2.2.\\\vspace{-0.12in}

\noindent \textbf{Response}: Self-supervised learning (SSL) has emerged as a powerful technique for various recommendation tasks with effective generative or contrastive data augmentation. Generally speaking, generative SSL recommenders~\cite{zhou2020s3,yuan2021improving} aim to learn a generative model for data reconstruction or imitation. Contrastive SSL models~\cite{wu2021self,xia2022hypergraph} use supervised contrastive loss by contrasting positive and negative samples. \\\vspace{-0.1in}

\noindent \textbf{\bf Response to Reviewer \#3} \\\vspace{-0.12in}

\noindent Thank you for the feedback and constructive suggestions. We have proofread our paper and corrected the identified typos. \\\vspace{-0.12in}

\noindent \textbf{Comment 1}: Clarification of hidden dimensionality $d$.\\\vspace{-0.12in}

\noindent \textbf{Response}: $d$ represents the embedding size for hidden states. \\\vspace{-0.12in}

\noindent \textbf{Comment 2}: Supplement the repository with evaluation data.\\\vspace{-0.12in}

\noindent \textbf{Response}: Due to file size limitations, we apologize for not including the experimental datasets in the anonymous repository. We have now uploaded all the experimental datasets together with detailed descriptions in compressed files to the repository, so they are fully available for reproducibility. \\\vspace{-0.12in}

\noindent \textbf{Comment 3}: Change of set definitions to tuples.\\\vspace{-0.12in}

\noindent \textbf{Response}: Thank you for bringing this to our attention. We have revised the text to correctly define user-item interaction, user-social interaction, and user-user interaction graphs as tuples, rather than sets in Section 2.1. \\\vspace{-0.12in}

\noindent \textbf{\bf Response to Reviewer \#4} \\\vspace{-0.12in}

\noindent Thank you for your valuable feedback. We have thoroughly revised our paper based on your comments and suggestions.

\noindent \textbf{Comment 1}: How social connections are established.\\\vspace{-0.15in}

\noindent \textbf{Response}: The social connections are provided by the collected datasets. Platforms (\eg, Ciao, Epinions and Yelp) allow users to establish social connections with each other and share reviews and ratings of products. Both user-item interactions and social network information are contained, but are presented in an anonymous format due to privacy. \\\vspace{-0.12in}

\noindent \textbf{Comment 2}: Further technical implementation details.\\\vspace{-0.12in}

\noindent \textbf{Response}: The embeddings of all methods are initialized using Xavier initialization. Moreover, early stop is utilized for model training. In order to prevent overfitting during model training, we implement dropout with a fixed ratio of 0.5. We have also set the negative slope for LeakyReLU as 0.5. \\\vspace{-0.12in}

\noindent \textbf{Comment 3}: \model's capability in handing heterophilic.\\\vspace{-0.12in}

\noindent \textbf{Response}: Our model \model\ can effectively handle the case where two connected users have opposite preferences. It can automatically align the social and interaction views to denoise the cross-view representation. The user-wise dependency weights learned by our model can be used to discover relation heterophily among users with adaptive SSL signals.







